Quantifying Jitter Transfer for Differential Measurement: Enhancing Security of Oscillator-Based TRNGs

The aim of this paper is to describe a way to improve the reliability of the measurement of the statistical parameters of the phase noise in a multi-ring oscillator-based TRNG. This is necessary to guarantee that the entropy rate is within the bounds prescribed by standards or security specifications. According to the literature, to filter out global noises which may strongly affect the measurement of the phase noise parameters, it is necessary to perform a differential measure. But a differential measurement only returns the parameters of the phase noise resulting of the composition of the noises of two oscillators whereas jitters parameters of individual oscillators are required to compute the entropy rate of a multi-ring oscillator-based TRNG. In this paper, we revisit the "jitter transfer principle" in conjunction with a tweaked design of an oscillator based TRNG to enjoy the precision of differential measures and, at the same time, obtain jitter parameters of individual oscillators. We show the relevance of our method with simulations and experiments with hardware implementations.

==> abstract.tex <==
On Jitter Transfer in Ring Oscillators

(joint work with David Lubicz)

Jitter in freely running ring oscillators serves as a crucial source of entropy, enabling the construction of \textbf{provably secure True Random Number Generators (TRNGs)}, backed by well-established stochastic models. To improve the quality and accuracy of entropy estimation—such as by mitigating global noise—ring oscillators are typically coupled. However, the stochastic dynamics of coupled systems are inherently complex and, until now, have been understood only approximately.

This talk will focus on \textbf{jitter transfer}, a heuristic approach for analyzing coupled noisy oscillators, where one oscillator is jitter-free and the other is jitter-compensated. I will present an \textbf{analytical solution} for the relative stochastic dynamics of coupled ring oscillators, providing a formal justification for the \textbf{jitter transfer principle}. These insights enable more accurate \textbf{jitter estimation} in multi-ring oscillator systems, resulting in enhanced TRNG performance.


